S3-DST: Structured Open-Domain Dialogue Segmentation and State Tracking in the Era of LLMs

The traditional Dialogue State Tracking (DST) problem aims to track user preferences and intents in user-agent conversations. While sufficient for task-oriented dialogue systems supporting narrow domain applications, the advent of Large Language Model (LLM)-based chat systems has introduced many real-world intricacies in open-domain dialogues. These intricacies manifest in the form of increased complexity in contextual interactions, extended dialogue sessions encompassing a diverse array of topics, and more frequent contextual shifts. To handle these intricacies arising from evolving LLM-based chat systems, we propose joint dialogue segmentation and state tracking per segment in open-domain dialogue systems. Assuming a zero-shot setting appropriate to a true open-domain dialogue system, we propose S3-DST, a structured prompting technique that harnesses Pre-Analytical Recollection, a novel grounding mechanism we designed for improving long context tracking. To demonstrate the efficacy of our proposed approach in joint segmentation and state tracking, we evaluate S3-DST on a proprietary anonymized open-domain dialogue dataset, as well as publicly available DST and segmentation datasets. Across all datasets and settings, S3-DST consistently outperforms the state-of-the-art, demonstrating its potency and robustness the next generation of LLM-based chat systems.

==> 03prompt_temp.tex <==
Real-world dialogues often exhibit extensive discourse that extends over multiple conversational turns in order to discuss diverse topics. This prolonged conversational nature makes it highly challenging to track contextual coherence. Previous studies \cite{hu-etal-2022-context} aimed at disassociating individual dialogue turns and processing them turn-by-turn for tracking dialogue state changes which worked reasonably well in task-oriented dialogues confined within predefined narrow domains. Nonetheless, real-world dialogues commonly require multiple turns to adequately comprehend the contextual nuances. Unfortunately, contemporary transformer-based models encounter challenges when processing lengthy input contexts, particularly in the middle \cite{liu2023lost} making it very difficult to track conversational states while maintaining context. To address these difficulties, we propose a novel turn-by-turn prompting technique that gives structure to inputs and outputs while accurately preserving the context in the process. We discuss these design aspects of our prompts below: 

\subsection{Structured Input and Output Formatting}
\label{method:xml}

\paragraph{Structured Input} For prompting LLMs, although it is trivial to channel plain conversation history in a flat format for analysis and inference, the unstructured nature inherent to this linear configuration makes it difficult to refer back and leverage different information across multiple conversational turns. To handle this challenge, we propose a structured inputting format, where each conversational history is formed into a hierarchical XML format where conversational turns are marked with turn id number \texttt{<T_id> .... </T_id>} numbered from $1$ to $N$ and each conversational turn consists of user and agent turns marked with appropriate XML tags (\texttt{<user>...</user>} and \texttt{<agent>...</agent>}. 

Since we propose instructing LLMs to infer binary (segment boundaries) and categorical labels (state values) per turn during our output, this input scheme helps us accurately refer back to the input turn and thus maintain coherence even for long dialogue contexts. Consistent with this XML-tagged input format, we also format all the valid segment and state (intent and domain) categories in an XML-formatted list. Empirically, this structured input and prompt formatting help constrain the LLM generation to follow the labeling instructions. Figure \ref{fig:s3-dst}(i) shows this format where each valid segment boundary and state category are first staged in an XML-formatted list and subsequently input dialogue is shown in a hierarchical configuration.

\paragraph{Structured Output} Our goal is a set of labels per dialogue turn representing the segment boundaries (binary labels) and state values (categorical labels). We propose to instruct the LLM to generate outputs in a hierarchical XML format. More specifically, we use a hierarchical XML format in which each turn, numbered from $T1$ to $TN$ comprises XML tree with several nested XML tags within it. The labels of these nested tags (e.g. \texttt{<preceding_topical_relation>...</preceding_topical_relation>}, \texttt{<segment_intent>...</segment_intent>}, and \texttt{<segment_domain>...</segment_domain>}  in Figure~\ref{fig:s3-dst}(ii)) represents a segment boundary or slot, and each value between opening and closing tags represent the model's inferred value. This is beneficial from two fronts: (i) Due to bounded well-defined structured formatting, generated outputs are more likely to be aligned with labeling instructions than free-form texts, and (ii) Well-formed structured output formats are easier to parse and reduce postprocessing requirements.

As a reminder, our target is a set of labels per dialogue turn representing the segment boundaries (binary labels) and state values (categorical labels).
Because this is a classification rather than generation task, we propose to instruct the LLM to format its output in a hierarchical structured manner.
Anecdotally, this approach helps constrain the LLM's generations to follow the labeling instructions and reduces postprocessing requirements.

Specifically, we use a hierarchical XML format in which each turn, numbered from 1 to $N$, comprises an XML tree with several nested XML tags within it.
These labels of these nested tags (e.g., ``preceding-topical-relation'', ``intent'' in Figure~\ref{fig:s3-dst}) represents a segment boundary or slot, and each value between the opening and closing tags represents the model's predicted value. 

To match this structured output format, we use  a structured prompt template approach as input to the LLM. 
Specifically, we provide all segment boundary classes and slot values as nested XML trees, with the class name as the top-level tag and all classes and their descriptions within each top-level tag. 
We also convert the dialogue from a raw text string to an XML-structured representation, with each user-agent turn nested between a turn-level tag.

\subsection{Pre-Analytical Recollection (PAR)}
\label{method:par}


As previously discussed, open-domain dialogues may be long and highly varied in conversation flow.
Therefore, it is crucial to ensure that the LLM can accurately track the dialogue context as it changes without forgetting or hallucination. 
To this end we propose Pre-Analytical Recollection (PAR), a strategy for turn-by-turn prompting that instructs the LLM to first summarize the turn within the top-level XML tag in 3 sentences or fewer \emph{before} providing the segment and state values. 
PAR is inspired by chain-of-thought prompting~\cite{wei2022chain}, as it is likewise a technique for generating intermediary relevant outputs in order to improve reasoning accuracy. 
In the context of dialogue systems, PAR is to force the model to ``recall'' the specific turn context before providing the labels, essentially grounding its classifications in the relevant conversation context.




\subsection{Final Prompt Configuration}
\label{method:prompt}

The final prompt flow of \method{} is provided in Figure~\ref{fig:s3-dst}. 
Given a raw conversation and a predefined set of segment and state labels,
we insert the labels into a structured prompt template and format the conversation in a hierarchical XML-structured representation.
We pass the prompt through the LLM, instructing it to follow PAR before jointly generating the hierarchical turn-by-turn segmentation and state labels.
